Generalization in Automated Process Discovery: A Framework based on Event Log Patterns

The importance of quality measures in process mining has increased. One of the key quality aspects, generalization, is concerned with measuring the degree of overfitting of a process model w.r.t. an event log, since the recorded behavior is just an example of the true behavior of the underlying business process. Existing generalization measures exhibit several shortcomings that severely hinder their applicability in practice. For example, they assume the event log fully fits the discovered process model, and cannot deal with large real-life event logs and complex process models. More significantly, current measures neglect generalizations for clear patterns that demand a certain construct in the model. For example, a repeating sequence in an event log should be generalized with a loop structure in the model. We address these shortcomings by proposing a framework of measures that generalize a set of patterns discovered from an event log with representative traces and check the corresponding control-flow structures in the process model via their trace alignment. We instantiate the framework with a generalization measure that uses tandem repeats to identify repetitive patterns that are compared to the loop structures and a concurrency oracle to identify concurrent patterns that are compared to the parallel structures of the process model. In an extensive qualitative and quantitative evaluation using 74 log-model pairs using against two baseline generalization measures, we show that the proposed generalization measure consistently ranks process models that fulfil the observed patterns with generalizing control-flow structures higher than those which do not, while the baseline measures disregard those patterns. Further, we show that our measure can be efficiently computed for datasets two orders of magnitude larger than the largest dataset the baseline generalization measures can handle.

==> tex/ConcurrentPatterns.tex <==
%!TEX root = ../journal_paper.tex
\newcommand{\outVertices}{\mathit{U}}
\newcommand{\compPartialFulfilment}{\mathit{computeFulfilmentWPartialMatching}}
\newcommand{\compInterleavingsFulfilment}{\mathit{computeFulfilmentWInterleavingsMatching}}
\newcommand{\usePartialMatching}{\mathit{usePM}}
\newcommand{\universeConcPatterns}{\mathcal{U}_{\Patterns,\mathit{conc}}}
\newcommand{\MT}{\mathit{MT}}
\newcommand{\LH}{\mathit{LH}}

\subsection{Identifying and measuring fulfilment of concurrent patterns}\label{sec:ConcPatternsFulfilment}

When activities occur in different orders in an event log, it induces that these activities can be executed concurrently in the underlying process. Further, in future traces we might observe more different orders of activities that can be derived from a concurrency oracle. All concurrent behavior inherent in an event log can be captured by the means of its partial orders. This concurrent behavior should be generalized in a process model by the means of parallel structures. Hence, we aim to identify and define concurrent patterns from the partial orders of an event log and then test them against the process model. For the concurrent patterns, we propose two ways of testing their partial fulfilment, i.e. if the process model contains a parallel structure for a subset of the concurrent activities.

The identification and definition of concurrent patterns relies on the partial orders constructed for a given event log and a concurrency oracle as described in Sec.~\ref{sec:Concurrency}. These partial orders represent relaxed orders of the traces of an event log incorporating the concurrency relations identified by the concurrency oracle. In order to test the concurrency captured in the relaxed orders, we will derive a set of representative traces with strict orders that represent all possible interleavings of each partial order. 
A concurrent pattern contained in a partial order always occurs at the same positions in all representative traces and represents all possible orderings of the concurrent activities. 
Hence, we define a concurrent pattern as a set of trace positions that is valid for all representative traces of a partial order. In addition, a concurrent pattern uses the trace count of the partial order as its weight and its partial fulfilment
measures the fraction of representative traces, in which the process model can match all or a subset of the concurrent activities at the trace positions of the pattern.
A partial order may define multiple concurrent patterns and relates to its set of representative traces. 
Formally, we define concurrent patterns and auxiliary functions next.

\begin{definition}[Concurrent patterns, Representative traces]
Given a partial order $\po$, a concurrent pattern $\concPattern$ is a tuple $\concPattern=(\tracePos,\traceCount,\partialFulfilment)$, where $
\tracePos$ is a set of trace positions of the representative traces of $\po$, $\traceCount$ is the trace count of the pattern and $\partialFulfilment$ is the partial fulfilment of the pattern. $\universeConcPatterns$ denotes the universe of concurrent patterns.
Additionally, we define functions $\concPatterns : \universePO\rightarrow\powerSet(\universeConcPatterns)$ and $\repTraces : \universePO\rightarrow\universeTraces$ that relate a partial order $\po$ to its set of concurrent patterns and representative traces, respectively.
\end{definition}

Given a partial order, we aim to identify its set of concurrent patterns and its set of representative traces with a breadth-first search over the partial order.
Since, we aim to extract strict orders of events for the representative traces from the partial order, we need to traverse a transitive reduction of the partial order.
The breadth-first search will traverse the partial order and collect events along the causality relations to iteratively construct its representative traces.
In particular, when an event with multiple outgoing events is encountered, the search will split into a construction of multiple traces, one for each outgoing event.
The traces are complete once the search encounters the final event of the partial order.
Concurrency in a partial order is captured as the absence of an arc between two events. 
Hence, if an event has multiple outgoing events in a transitively reduced partial order, these outgoing events are concurrent to each other. 
In fact, all events following the concurrent events are also concurrent until an event is reached with several incoming arcs that consolidates all paths starting from the event with multiple outgoing events.
The representative traces constructed by the search must include all concurrent events in between the event with multiple outgoing and the event with multiple incoming events to form a valid execution of a partial order.
The breadth-first search can consider concurrent events by traversing one outgoing event and then keeping all other outgoing events in a memory.
In every iteration, the search will then not only consider the outgoing events but also all events from the memory and the traversed event is removed from the memory.
In order to consolidate the concurrent paths, an event with multiple incoming events can only be traversed by the search, if a trace constructed by the search up to that point contains all its incoming events, i.e. all concurrent events have been traversed before the concurrent block of a partial order ends.
That way, the search can enumerate all orders of events in different traces from a concurrent block that starts with an event with multiple incoming and end with an event with multiple incoming arcs.
We also use this structure to define concurrent patterns during the search, i.e. we start a new concurrent pattern when we encounter an event with multiple outgoing events. 
The pattern will add the trace positions whenever the search adds concurrent events to the constructed trace until the search successfully traverses an event with multiple incoming events and the memory is empty. In that case, the search completes the definition of the concurrent pattern as the set of recorded trace positions and the trace count of the partial order. The partial fulfilment of the pattern needs to be determined after all representative traces for the partial order have been computed. 

%\newpage
\begin{algorithm}[h!]
{
    \caption{Compute representative traces and concurrent patterns for partial orders}\label{alg:compRepTracesAndConcPatterns}    
    \SetKwInOut{Input}{input}
    \SetKwProg{Fn}{Function}{}{}
    \Input{Event log $\logL$; Concurrency oracle $\concOracle=(\conc,\xi)$;}
    $\repTraces\leftarrow\{\}$;
    $\concPatterns\leftarrow\{\}$\;
    \For{$\po=(\Events,\Causality,\poLabelling)\in\uniqueTraces(\xi(\logL))$}
    {      
        $\open\leftarrow\langle(\initialEvent,\langle\rangle,\{\},\{\},0)\rangle$\;
        \While{$\open\neq\varnothing$}{        
            $(v,t,\memory_v,\tracePos^v,\concurrent_v)\leftarrow\head(\open)$;
            $\open\leftarrow\tail(\open)$\;
            \lIf{$\left|(v,u)\in\Causality\right|>1$}{$\concurrent_v\leftarrow 1$}
            $\outVertices\leftarrow\{u\mid(v,u)\in\Causality\lor u\in\memory_v\}$\;
            \For{$u\in\outVertices$}{
                \If{$\forall (w,u)\in\Causality : w\in t$}{
                    \lIf{$u=\finalEvent$}{$\repTraces(\po)\leftarrow\repTraces(\po)\cup\{\poLabelling(t)\}$}
                    \Else
                    {
                        $n_u\leftarrow(u,t_u\leftarrow t\concat u,\memory_u\leftarrow\memory_v\setminus\{u\},\tracePos^u\leftarrow\tracePos^v,\concurrent_u\leftarrow\concurrent_v)$\;
                        \If{$\left|(w,u)\in\Causality\right|>1\land\memory_u=\varnothing\land\tracePos^v\neq\varnothing$}{
                            $\concPatterns(\po)\leftarrow\concPatterns(\po)\cup\{\tracePos^v,\countTr(\po,\xi(\logL)),\perp\}$\;
                            $\tracePos^u\leftarrow\{\}$\;
                            $\concurrent_u\leftarrow 0$\;                    
                        }
                        \lIf{$\left|(v,w)\in\Causality\right|>1$}{
                            $\memory_u\leftarrow\memory_u\cup\{w\mid (v,w)\in\Causality\land w\neq u\land (x,w)\in\Causality\Rightarrow x\in t\}$                        
                        }
                        \lIf{$\concurrent_u=1$}{
                               $\tracePos^u\leftarrow\tracePos^u\cup\left|t_u\right|$                 
                        }    
                        $\open\leftarrow\open\concat n_u$\; 
                    }
                } 
            }
        }      
    }
    \Return{$\repTraces,\concPatterns$}\;
}
\end{algorithm}

Given an event log and a concurrency oracle, Alg.~\ref{alg:compRepTracesAndConcPatterns} computes functions relating each unique partial order of the event log to its set of representative traces and its set of concurrent patterns.
The breadth first search is conducted for each partial order via an open list $\open$ that stores nodes of the search as a quintuple $(v,t,\memory_v,\tracePos^v,\concurrent_v)$, which contains the current event $v$, the currently constructed trace of events $t$, the memory $\memory_v$ of a set of concurrent events that still need to be traversed, the trace positions of the current concurrent pattern $\tracePos^v$ and a boolean variable $\concurrent_v$ indicating if the current event is concurrent.
In every iteration of the search, the first node of the search is removed.
If the current event has multiple outgoing events, the search from the current node is set to concurrent, i.e. $\concurrent_v=1$.
Then, the search considers to traverse every event $u$ in the outgoing events of $v$ and from memory $\memory_v$, but only if every incoming event $w$ of $u$ is already traversed, i.e. $w\in t$.
If $u$ is the final event, the search will add the sequence of activity labels of all events of trace $t$ to the set of representative traces of the partial order and continues the search.
Otherwise, a new node for the search is created, where $u$ is the current event, trace $t$ adds event $u$, the memory carries over all events from $\memory_v$ besides $u$ and both $\tracePos^v$ and $\concurrent_v$ are carried over.
If $u$ closes a concurrent block of events, i.e. if it has multiple incoming events, the memory is empty and the set of trace positions is not empty, then we will add the concurrent pattern tracked with $\tracePos^v$ to the set of concurrent patterns of the partial order. Furthermore, the set of trace positions of the new node is emptied and $\concurrent_u$ is set to zero.
If the current event $v$ has multiple outgoing events, then the memory of the new node $\memory_u$ is extended by all outgoing events $w$ of $v$ that are not $u$ and for which all their incoming events are included in the trace $t$.
If the current node is concurrent, i.e. $\concurrent_v=1$, then we extend the set of trace positions $\tracePos^u$ by the position of the currently added event $u$, i.e. $\left|t_u\right|$.
Finally, the new node is added to the open list and the search continues until all possible orders of the partial order have been traversed and all representative traces as well as all concurrent patterns have been gathered.

The partial fulfilment of the identified patterns can only be determined after all representative traces for a partial order have been determined since the fulfilment relies on the alignments of the representative traces. 
In this article, we propose two ways of measuring the partial fulfilment of a concurrent pattern: one based on \emph{interleavings matching} and one based on \emph{partial matching}. 
The interleavings matching measures how many orders of the concurrent activities, aka. interleavings, can be fully matched by the process model. 
In particular, every ordering of the concurrent activities is captured in one of the representative traces and hence the fulfilment can be determined as the fraction of alignments that can align all trace positions of the concurrent patterns with matches.
The partial matching is a more lenient method in that it does not require full matches for each order of concurrent activities. Instead, it measures the fraction of the number of matches at the trace positions of the concurrent pattern for all representative traces against the overall number of trace positions of all traces.
The choice of matching method for concurrent patterns depends on the user's preferences of how strictly a concurrent pattern should be matched.
In general, the interleavings matching will produce generally lower and less diverse scores while partial matching will result in higher but more distinctive scores.
Alg.~\ref{alg:compPartialFulfilmentConcurrentPatterns} then shows the computation of the partial fulfilments for all concurrent patterns. The algorithm allows to select the matching method for computing partial fulfilments with the boolean $\usePartialMatching$. 

\begin{algorithm}[h]
{
    \caption{Compute partial fulfilments of concurrent patterns}\label{alg:compPartialFulfilmentConcurrentPatterns}    
    \SetKwInOut{Input}{input}
    \SetKwProg{Fn}{Function}{}{}
    \Input{Event log $\logL$; System net $\sysNet$; Concurrency oracle $\concOracle=(\conc,\xi)$; Representative Traces $\repTraces$; Concurrent pattern definitions $\concPatterns$; Use partial matching $\usePartialMatching$;}
    \For{$\po\in\uniqueTraces(\xi(\logL)$)}{
        $\alignments\leftarrow \text{align}(\repTraces(\po),\sysNet)$\;
        \For{$\concPattern\in\concPatterns(\po)$}{
            \uIf{$\usePartialMatching=1$}{
                 $\partialFulfilment(\concPattern)\leftarrow\compPartialFulfilment(\concPattern,\alignments)$\;
             }
             \Else{
                 $\partialFulfilment(\concPattern)\leftarrow\compInterleavingsFulfilment(\concPattern,\alignments)$\; 
             }       
        }    
    }
    \Return{$\concPatterns$}\;
    \Fn{$\compPartialFulfilment(\concPattern,\alignments)$}
    {
        $\partialFulfilment\leftarrow 0$\;
        \For{$\alignment\in\alignments$}{        
            $\alignmentTraceOps\leftarrow\op(\filterSyncDFA(\alignment))$\;
            $\partialFulfilment\leftarrow\partialFulfilment+\left|\{\pos\in\tracePos(\concPattern)\mid\alignmentTraceOps[\pos]=\match\}\right|$\;  
        }
        \Return{$\partialFulfilment/(\left|\tracePos(\concPattern)\right|*\left|\alignments\right|)$}\;    
    }
    \Fn{$\compInterleavingsFulfilment(\concPattern,\alignments)$}{
        $\partialFulfilment\leftarrow 0$\;
        \For{$\alignment\in\alignments$}{        
            $\alignmentTraceOps\leftarrow\op(\filterSyncDFA(\alignment))$\;
            \lIf{$\forall \pos\in\tracePos(\concPattern) : \alignmentTraceOps[\pos]=\match)$}{
                $\partialFulfilment\leftarrow\partialFulfilment+1$            
            } 
        }
        \Return{$\partialFulfilment/\left|\alignments\right|$}\; 
    }
}
\end{algorithm}

In summary, given an event log, a system net, a concurrency oracle and the option of a matching method, the concurrent patterns can be defined by:
\begin{inparaenum}[(1)]
    \item Building the partial orders for the unique traces of an event log via the concurrency oracle as described in Sec.~\ref{sec:Concurrency};
    \item Identifying the representative traces and concurrent patterns of each partial order with a breadth-first search of Alg.~\ref{alg:compRepTracesAndConcPatterns};
    \item Computing the partial fulfilments of all concurrent patterns based on the alignments of the representative traces and the system net via the selected matching method in Alg.~\ref{alg:compPartialFulfilmentConcurrentPatterns}.
\end{inparaenum}
We overload the notation of $\concPatterns$ to return a set of concurrent patterns for a given event log $\logL$ after applying all steps, i.e. $\concPatterns(\logL)=\{\repPatterns(\et)\mid\et\in\extLog\}$.

\begin{figure*}[h!]
\centering
\resizebox{1\textwidth}{!}{ 
 \tikzstyle{IDHL} = [draw, rectangle, fill=white, align=center, minimum height=5.5mm, text width={width("$t  (8),(9)  t$")}, font=\footnotesize]
 \tikzstyle{ID} = [draw, rectangle, fill=white, align=center, minimum height=31mm, text width={width("$t  (8),(9)  t$")}, font=\footnotesize]
 \tikzstyle{REPTRACE} = [draw, rectangle, fill=white, align=left, minimum height=5mm, text width={width("$t X,A,B,C t$")}, font=\footnotesize]
 \tikzstyle{REPALIGNMENT} = [draw, rectangle, fill=white, align=left, minimum height=5mm, text width={width("$t MT(X),MT(A),MT(B),MT(C)$")}, font=\footnotesize]
 \tikzstyle{CONCPATTERNHL} = [draw, rectangle, fill=white, align=left, minimum height=5mm, text width={width("$pf(pco)w.IMt$")}, font=\footnotesize]
 \tikzstyle{CONCPATTERN} = [draw, rectangle, fill=white, align=center, minimum height=31mm, text width={width("$pf(pco)w.IMt$")}, font=\footnotesize]
 \begin{tikzpicture}[>=stealth', node distance=-0.3pt]
  \node[IDHL] (id) {\bf{ID}};  
  \node[REPTRACE, right=of id] (repTraces) {\bf{$t\in\repTraces(\po)$}};
  \node[REPALIGNMENT, right=of repTraces] (repAlignments){\bf{$\alignment\in\text{align}(\repTraces(\po),\sysNet)$}};
  \node[CONCPATTERNHL, right=of repAlignments] (concPatternsTracePos){\bf{$\tracePos(\concPattern)$}};
  \node[CONCPATTERNHL, right=of concPatternsTracePos] (concPatternsSize){\bf{$\traceCount(\concPattern)$}};
  \node[CONCPATTERNHL, right=of concPatternsSize] (concPatternsPFIM){$\partialFulfilment(\concPattern)\text{ w.IMt}$};
  \node[CONCPATTERNHL, right=of concPatternsPFIM] (concPatternsPFPM){$\partialFulfilment(\concPattern)\text{ w.PMt}$};
  \node[ID, below=of id] (id12) {(1),(2)};
  \node[REPTRACE, below=of repTraces] (repTrace1) {$\langle X,A,B,C \rangle$};
  \node[REPTRACE, below=of repTrace1] (repTrace2) {$\langle X,A,C,B \rangle$};
  \node[REPTRACE, below=of repTrace2] (repTrace3) {$\langle X,B,A,C \rangle$};
  \node[REPTRACE, below=of repTrace3] (repTrace4) {$\langle X,B,C,A \rangle$};
  \node[REPTRACE, below=of repTrace4] (repTrace5) {$\langle X,C,A,B \rangle$};
  \node[REPTRACE, below=of repTrace5] (repTrace6) {$\langle X,C,B,A \rangle$};
  \node[REPALIGNMENT,below=of repAlignments] (repAlignment1) {$\langle \MT(X),\MT(A),\MT(B),\MT(C)\rangle$};
  \node[REPALIGNMENT,below=of repAlignment1] (repAlignment2) {$\langle \MT(X),\MT(A),\MT(C),\MT(B)\rangle$};
  \node[REPALIGNMENT,below=of repAlignment2] (repAlignment3) {$\langle \MT(X),\MT(B),\LH(A),\MT(C)\rangle$};
  \node[REPALIGNMENT,below=of repAlignment3] (repAlignment4) {$\langle \MT(X),\MT(B),\MT(C),\LH(A)\rangle$};
  \node[REPALIGNMENT,below=of repAlignment4] (repAlignment5) {$\langle \MT(X),\MT(C),\LH(A),\MT(B)\rangle$};
  \node[REPALIGNMENT,below=of repAlignment5] (repAlignment6) {$\langle \MT(X),\MT(C),\MT(B),\LH(A)\rangle$};
  \node[CONCPATTERN, below=of concPatternsTracePos] (concPatternsTracePos1){$\{2,3,4\}$};
  \node[CONCPATTERN, right=of concPatternsTracePos1] (concPatternsTraceCount1){$2000$};
  \node[CONCPATTERN, right=of concPatternsTraceCount1] (concPatternsPFIM1){$2/6$};
  \node[CONCPATTERN, right=of concPatternsPFIM1] (concPatternsPFPM1){$14/18$};
  \end{tikzpicture}
  }
 \caption{Representative traces and concurrent patterns for the partial order $\po$ of the running example from Fig.~\ref{fig:PO_TransitiveReduction}.}\label{fig:runningExampleConcPatterns}
\end{figure*}

Fig.~\ref{fig:runningExampleConcPatterns} shows the representative traces and concurrent patterns for traces with identifiers (1) and (2) from the running example log of Fig.~\ref{fig:runningExampleLog}. Both traces map to the same partial order $\po$ from Fig.~\ref{fig:PO_TransitiveReduction}. When applying Alg.~\ref{alg:compRepTracesAndConcPatterns} to $\po$, we can derive six representative traces $\repTraces(\po)$ enumerating all orders of concurrent activities $A$,$B$ and $C$ after executing $X$. The column to the right shows the alignments for the representative traces with the system net $\sysNet$ from the running example in Fig.~\ref{fig:runningExampleModel}. 
The algorithm identifies one concurrent pattern spanning trace positions 2,3 and 4 of all representative traces and has a trace count of 2000, i.e. summing up the trace counts from traces (1) and (2).
Applying Alg.~\ref{alg:compPartialFulfilmentConcurrentPatterns} with interleavings matching (short w.IMt), the concurrent pattern can match all three concurrent activities in only two out of six alignments.
For partial matching (short w.PMt), the concurrent pattern can match in total 14 out of 18 alignment steps corresponding to the three positions of the pattern over all six of the alignments.
Both matching methods identify that the system net does not model the three concurrent activities with a parallel block. 
Interleavings matching assigns a lower score of fulfilment since only two orders can be fulfilled by the model, while the partial matching rewards the fact that activities $B$ and $C$ are concurrent in the model.



==> tex/ProofExactExtendedAlignments.tex <==
% !TEX root = ../journal_paper.tex
%\todo[inline, color=red]{I propose the following structure:}

%\todo[inline, color=yellow]{I think it is better to separate the results where $\costF(\extalignment)=\costF(\alignment)$, as those results are not about the over-approximation. @Daniel, make the corresponding adjustments please.}

\begin{proof}[sketch]
\begin{enumerate}
\item First, let $t$ contain \emph{no tandem repeats}. In that case, after applying Alg.~\ref{alg:reduceLog}, the reduced trace $rt$ will be the same as trace $t$. The algorithms for computing alignments for reduced traces (Alg.~\ref{alg:BinarySearchAlignments}) and to compute optimal alignments (Alg.~\ref{alg:fsmAlignments}) differ only in their cost function. The reduced cost function (Def.~\ref{def:adjustedCostF}) assigns different costs to alignment synchronizations corresponding reduced tandem repeats. Hence, in the absence of tandem repeats, the cost functions are effectively the same. Hence, it follows that an extended alignment for $t$ without tandem repeats will achieve the same cost as an optimal alignment, i.e. $\costF(\extalignment)=\costF(\alignment)$.
% Alg.~\ref{alg:BinarySearchAlignments} will compute an alignment $\redalignment$ for $rt$ with the same cost as $\alignment$. Applying the ezxtension algorithm~\ref{alg:ExtendRedAlignments} will result in the same alignment as $rt$ does not contain tandem repeats that could be extended. It follows that an extended alignment for $t$ without tandem repeats will achieve the same cost as an optimal alignment, i.e. $\costF(\extalignment)=\costF(\alignment)$.

\item $t$ contains a single tandem repeat $(i,\alpha,k)$. The tandem repeat will be reduced to two copies (Alg.~\ref{alg:reduceLog}) in a reduced trace $rt$. The main difference for computing the alignments for $rt$ lies in the selection of synchronizations with the use of the adjusted cost function from Def.~\ref{def:adjustedCostF}. 
%We already established that Alg.~\ref{alg:BinarySearchAlignments} selects synchronizations similarly to Alg.~\ref{alg:fsmAlignments} for synchronizations outside of a tandem repeat. 
The selection of synchronizations for a tandem repeat does not change the selection of synchronizations outside the tandem repeat since the accumulated cost of aligning a tandem repeat according to the adjusted cost function is the same as aligning the tandem repeat in $t$ with Alg.~\ref{alg:fsmAlignments}, which has been shown in the proof in \ref{app:proof_costFrelation}. Hence, we only need to investigate whether aligning the tandem repeat and its extension will lead to an over-approximation of the alignment cost of $\extalignment$.
For that we need to consider how the tandem repeat can be aligned to $\reachGraph$:

\begin{enumerate}
	\item First, we consider a \emph{tandem repeat with no possible matches}, i.e. the reachability graph $\reachGraph$ does not contain any arcs with labels of $\alpha$ such that $l\in\alpha\Rightarrow(n_s,l,n_t)\notin\rgArcs$. In that case, an optimal alignment $\alignment$ will hide all trace labels related to the tandem repeat. A reduced alignment $\redalignment$ will hide all trace labels of the two copies of the reduced tandem. The extension from Alg.~\ref{alg:ExtendRedAlignments} will identify no label that has been aligned with a $\match$ operation in both copies and hence the middle copy will consist of all hide operations. The middle copy will be used to recreate the $k$ repetitions and as a result $\extalignment$ will have the same cost as $\alignment$ with no over-approximation, i.e. $\costF(\extalignment)=\costF(\alignment)$.
	
	\item Second, we consider a \emph{tandem repeat with no corresponding loop in the model}. It follows that every label of the repeating sequence $\alpha$ can be matched at most once since a label matching in two repetitions would establish a loop in the reachability graph.  An optimal alignment $\alignment$ could then match each of the labels of the repeating sequence once in arbitrary repetitions. The reduced alignment $\redalignment$ can also match  each label of the repeating sequence once in one of the two maintained repetitions. The middle copy would again consist of all hide operations and hence the extended alignment $\extalignment$ can also achieve the same cost as $\alignment$ without over-approximation, i.e. $\costF(\extalignment)=\costF(\alignment)$.
	
	\item Next, we consider a \emph{tandem repeat with all matches}, i.e. its labels can be perfectly matched to a loop in the reachability graph. In that case, the optimal alignment $\alignment$ will align all trace labels corresponding to the tandem repeat with $\match$ operations. The reduced alignment $\redalignment$ can similarly match both repetitions of the reduced tandem repeat since there exists a loop in the reachability graph with the labels of the tandem repeat. The extension algorithm~\ref{alg:ExtendedRedAlignments} will identify a repeating sequence at the first label of the repeating sequence with a $\match$ operation in both repetitions. The middle copy inserted to recreate $k$ repetitions then consists of all $\match$ synchronizations since both repetitions of the tandem repeat could be matched in $\redalignment$. Hence, $\extalignment$ will consist of all $\match$ synchronizations for the tandem repeat and has the same cost as $\alignment$ with no over-approximation, i.e. $\costF(\extalignment)=\costF(\alignment)$.
\end{enumerate}

\end{enumerate}

\end{proof}

==> tex/figureAAdataset.tex <==
%!TEX root = ../Appendix.tex
\begin{figure}[!h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\resizebox{0.66\textwidth}{!}{ 
 \tikzstyle{ID} = [draw, rectangle, fill=white, align=center, minimum height=5mm, text width={width("$t  (1)  t$")}, font=\footnotesize]
 \tikzstyle{TRACE} = [draw, rectangle, fill=white, align=left, minimum height=5mm, text width={width("$t A,C,D,G,H,F,I t$")}, font=\footnotesize]
 \tikzstyle{COUNT} = [draw, rectangle, fill=white, align=center, minimum height=5mm, text width={width("$t count(dt,L) t$")}, font=\footnotesize]
 \begin{tikzpicture}[>=stealth', node distance=-0.3pt]
  \node[TRACE] (log) {\bf{$dt\in\uniqueTraces(\logL)$}};
  \node[ID, left=of log] (id) {\bf{ID}};
  \node[COUNT, right=of log] (count){\bf{$\countTr(dt,\logL)$}};
  \node[TRACE, below=of log] (trace1) {$\langle A,B,D,E,I \rangle$};
  \node[ID, left=of trace1] (id1) {(1)};
  \node[COUNT,right=of trace1] (count1) {1207};
  \node[TRACE, below=of trace1] (trace2) {$\langle A,C,D,G,H,F,I \rangle$};
  \node[ID, left=of trace2] (id2) {(2)};
  \node[COUNT,right=of trace2] (count2) {145};
  \node[TRACE, below=of trace2] (trace3) {$\langle A,C,G,D,H,F,I \rangle$};
  \node[ID, left=of trace3] (id3) {(3)};
  \node[COUNT,right=of trace3] (count3) {56};
  \node[TRACE, below=of trace3] (trace4) {$\langle A,C,H,D,F,I \rangle$};
  \node[ID, left=of trace4] (id4) {(4)};
  \node[COUNT, right= of trace4] (count4) {23};
  \node[TRACE, below=of trace4] (trace5) {$\langle A,C,D,H,F,I \rangle$};
  \node[ID, left=of trace5] (id5) {(5)};
  \node[COUNT, right= of trace5] (count5) {28};
  \end{tikzpicture}
  }
 \caption{Original Event log of AA dataset.}\label{fig:AA_Log_original}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.85\textwidth]{Figures/GeneratingModel.png}
    %\vspace{-.5\baselineskip}
    \caption{Generating Model} \label{fig:AA_GeneratingModel}
    \vspace{\baselineskip}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.85\textwidth]{Figures/SingleTraceModel.png}
  %\vspace{-.5\baselineskip}
  \caption{Single Trace Model} \label{fig:AA_SingleTraceModel}
  %\vspace{-2\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/FlowerModel.png}
  %\vspace{-.5\baselineskip}
  \caption{Flower Model} \label{fig:AA_FlowerModel}
  \vspace{\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{Figures/SeparateTracesModel.png}
    %\vspace{-.5\baselineskip}
    \caption{Four distinct traces Model} \label{fig:AA_DistinctTracesModel}
    %\vspace{-2\baselineskip}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/GH_Parallel_Model.png}
  %\vspace{-.5\baselineskip}
  \caption{G and H parallel Model} \label{fig:AA_GH_Parallel_Model}
  %\vspace{\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/GH_SelfLoop_Model.png}
  %\vspace{-.5\baselineskip}
  \caption{G and H in self loops Model} \label{fig:AA_GH_SelfLoop_Model}
  %\vspace{-2\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/D_SelfLoop_Model.png}
  %\vspace{-.5\baselineskip}
  \caption{D in a self loop Model} \label{fig:D_SelfLoop_Model}
  %\vspace{-2\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.6\textwidth]{Figures/AllParallelModel.png}
  %\vspace{-.5\baselineskip}
  \caption{All parallel Model} \label{fig:AA_AllParallelModel}
  \vspace{\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/RoundRobinModel.png}
  %\vspace{-.5\baselineskip}
  \caption{Round Robin Model} \label{fig:AA_RoundRobinModel}
  %\vspace{-2\baselineskip}
  %\caption{Concurrencies from the local oracle}
  %\label{fig:sub2}
\end{subfigure}%
\caption{Event Log and Process models of the AA dataset from~\cite{AntiAlignments}}
\label{fig:DatasetAA}
\end{figure}
